Multi-task Learning for Joint Re-identification, Team Affiliation, and Role Classification for Sports Visual Tracking

Effective tracking and re-identification of players is essential for analyzing soccer videos. But, it is a challenging task due to the non-linear motion of players, the similarity in appearance of players from the same team, and frequent occlusions. Therefore, the ability to extract meaningful embeddings to represent players is crucial in developing an effective tracking and re-identification system. In this paper, a multi-purpose part-based person representation method, called PRTreID, is proposed that performs three tasks of role classification, team affiliation, and re-identification, simultaneously. In contrast to available literature, a single network is trained with multi-task supervision to solve all three tasks, jointly. The proposed joint method is computationally efficient due to the shared backbone. Also, the multi-task learning leads to richer and more discriminative representations, as demonstrated by both quantitative and qualitative results. To demonstrate the effectiveness of PRTreID, it is integrated with a state-of-the-art tracking method, using a part-based post-processing module to handle long-term tracking. The proposed tracking method outperforms all existing tracking methods on the challenging SoccerNet tracking dataset.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*


.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> samples/Sections/introduction_old.tex <==
Soccer is one of the most popular sports worldwide, attracting millions of fans and players alike. With the proliferation of video technology, it has become possible to track and analyze players' movements on the field. This has led to a growing interest in developing computer vision techniques for player tracking and re-identification in soccer videos. These techniques have potential applications in a variety of areas, such as sports broadcasting \cite{vats2023player}\cite{tong2011automatic}, coaching \cite{chen2016learning}\cite{thomas2017computer}, and performance analysis \cite{darwish2022ste}\cite{uchida2021automated}\cite{istasse2019associative}\cite{theagarajan2020automated}.

While recent work in pedestrian tracking has shown promising results by formulating multi-target tracking in terms of data association \cite{bewley2016simple}\cite{wojke2017simple}\cite{aharon2022bot}\cite{zhang2022bytetrack}\cite{du2023strongsort}\cite{cao2023observation}, player tracking in team sports presents unique challenges due to non-linear player motion, similar appearances of players on the field, and frequent occlusions. These challenges make it difficult to accurately track and re-identify players throughout the game. Therefore, re-identification plays a crucial role in player tracking and can significantly impact the accuracy of tracking methods. By accurately re-identifying players in soccer videos, tracking them becomes much easier. Although there has been a lot of research on re-identifying pedestrians \cite{fan2019spherereid}\cite{luo2019bag}, recently, part-based re-identification methods have gained attention due to their potential to localize different parts of a person and identify individuals using these parts \cite{sun2018beyond}\cite{xu2021dual}\cite{somers2023body}. These methods have shown promising results in dealing with the challenges such as occlusions. In addition, there have been several works that specifically focus on tracking and re-identification in sports \cite{liu2020part}\cite{maglo2022efficient}\cite{zhang2020multi}\cite{scott2022soccertrack}. However, a major challenge in this area has been the lack of a common dataset for evaluating and comparing different tracking and re-identification methods. To address this issue, the recently-introduced SoccerNet-Tracking dataset provides a common benchmark for evaluating player tracking and re-identification methods in soccer videos \cite{cioppa2022soccernet}.

 In this work, the potential of part-based re-identification in improving tracking results on the SoccerNet-Tracking dataset is investigated. Specifically, a recent part-based re-identification method called BPBReID \cite{somers2023body} is utilized, and two new objectives are added to the model, including team affiliation and role classification. The model is trained jointly for person re-identification, team affiliation, and role classification to create more meaningful part-based embeddings for players. To integrate part-based features into the tracking process, a recent appearance-based tracking method called Strong-SORT \cite{du2023strongsort} is used. Additionally, a post-processing step with part-based features is proposed to merge unmatched tracklets. To evaluate tracking on soccer videos, the SoccerNet-Tracking dataset is used. Finally, to train and evaluate the re-identification model, a re-identification dataset is created from SoccerNet-Tracking videos.


In summary, the main contributions of this work are as follows:
\begin{itemize}

\item Utilizing a part-based re-identification method (BPBReID) and adding two new objectives to the model for joint training for re-identification, team affiliation, and role classification.

\item Proposing a part-based tracking method by integrating pbart-based features to the one of the state-of-the-art tracking methods, Strong-SORT, and adding a postprocessing step using part-based features.

\item Creating a re-identification dataset from tracking dataset for training and evaluating re-identification model.

\item Validating the effectiveness of the proposed methods by evaluating the performance of the part-based ReID model on the proposed ReID dataset and comparing tracking results with some existing tracking methods on the SoccerNet-Tracking dataset.


\end{itemize}




==> samples/Sections/introduction_v2_Amir.tex <==
Soccer is one of the most popular sports worldwide, attracting millions of fans and players alike. With the proliferation of video technology, it has become possible to track and analyze players' movements on the field. Automated sport analysis involves the use of computer vision and deep  learning techniques to analyze sports events and extract meaningful insights and has potential applications in a variety of areas, such as sports broadcasting \cite{vats2023player, tong2011automatic}, coaching \cite{chen2016learning, thomas2017computer}, and performance analysis \cite{darwish2022ste, uchida2021automated, istasse2019associative, theagarajan2020automated}. One of the key components of automated sport analysis is object tracking, which involves the identification and tracking of players and objects in a video. Tracking is essential for automated sport analysis for three main reasons. Firstly, it allows for the identification and distinction of players and objects, enabling the extraction of useful information such as speed, distance, and key events. Secondly, it creates a spatio-temporal representation of the game, providing a detailed overview that can identify patterns and trends. Lastly, tracking reduces the manual effort required for analysis, allowing analysts to focus on higher-level tasks. 

Tracking is the process of identifying and following objects of interest in a video, which is challenging due to complex and dynamic motion, occlusions, appearance variations, and real-time processing requirements. Re-identification, on the other hand, is a powerful tool for solving the tracking task because it captures the appearance of an object, such as a player, which allows the tracker to continue following the object even when it becomes occluded or moves out of the camera's field of view. By incorporating appearance-based methods such as re-identification, the likelihood of losing the track of an object is reduced, leading to improved tracking performance. However, combining tracking and re-identification with team and role information provides a more comprehensive understanding of the game, allowing for more detailed and accurate automated sport analysis.

Despite the significant progress in tracking methods for sports analysis \cite{lu2013learning, hurault2020self, yang2021multi, maglo2022efficient}, most current methods in the literature do not solve all tasks, such as tracking, re-identification, team and role identification, simultaneously, and often require multiple networks with independent backbones, which are computationally expensive and suboptimal, since all three tasks concern sport person representation and are closely related, which may cause issues for real-time applications. This is evident from the large number of sport tracking papers that focus on one or two tasks, such as tracking and re-identification, while leaving out team and role identification, or vice versa. The role classification task is typically accomplished by the upstream object detector, but most state-of-the-art pre-trained detectors are limited to the "person" class and cannot distinguish between various sports roles (player, goalkeeper, referee, staff, etc). Similarly, the team affiliation task is often incorrectly formulated as a classification task with predefined teams \cite{vats2023player}, which can cause issues if two different teams use similar jerseys. Moreover, Re-Identification (ReID) models trained solely with identity labels may not be suitable for team affiliation tasks, as they may consider players with similar attributes, such as skin color, more similar to each other than players from the same team, resulting in inaccurate team identification.

To address the aforementioned issues, we propose a novel sports person representation model that generates a multi-purpose representation from a single backbone, enabling the joint solving of person re-identification, team affiliation, and role classification tasks. Our method has two key benefits: first, by integrating three distinct representation objectives during training, the model generates richer representations, resulting in superior re-identification performance compared to models trained with a single objective; second, it is computationally efficient as it jointly solves three tasks using a single backbone.

%Different from previous works, where team affiliation is formulated as a classification task, our model formulates it as a deep metric learning task, allowing it to generalize to any team and distinguish between two teams it has not seen during training.

In this work, a state-of-the-art body part-based re-identification model, BPBreID\cite{somers2023body}, is used as the base of our joint model. Two new heads are then added to this network: role classification and team affiliation. The role head performs a classification task to specify the role of each person, while the team affiliation task is a re-identification-like task on the team identity of the players with a subsequent clustering for specifying team labels. A multi-task approach is utilized to train the model jointly for all three tasks, resulting in an embedding for each part of the body of a person which is used to solve the three tasks at inference. This method is called PRTreID (Part-based Role Team reidentification) in this paper.

Furthermore, our proposed PRTreID model is integrated with a state-of-the-art re-identification-based tracking method, namely StrongSORT. We also replace the post-processing step of this tracker with our proposed part-based tracklet merging module and introduce our PRT-Track method for tracking persons in soccer videos.

In summary, the main contributions of this work are as follows:
\begin{itemize}

\item Utilizing a part-based re-identification method (BPBReID) and adding two new objectives to the model for joint training for re-identification, team affiliation, and role classification.

\item Proposing a part-based tracking method by integrating part-based features to the one of the state-of-the-art tracking methods, Strong-SORT, and adding a postprocessing step using part-based features.

\item Validating the effectiveness of the proposed methods on the SoccerNet-Tracking dataset.


\end{itemize}




==> samples/Sections/introduction_vladimir.tex <==
                    %%%%%%%%%%%%%%%%%%%%%%%%%%
%-------------------%        OVERVIEW        %--------------------
                    %%%%%%%%%%%%%%%%%%%%%%%%%%
General overview of automated sport analysis, previous text was ok
% Soccer is one of the most popular sports worldwide, attracting millions of fans and players alike. With the proliferation of video technology, it has become possible to track and analyze players' movements on the field. This has led to a growing interest in developing computer vision techniques for player tracking and re-identification in soccer videos. These techniques have potential applications in a variety of areas, such as sports broadcasting \cite{vats2023player}\cite{tong2011automatic}, coaching \cite{chen2016learning}\cite{thomas2017computer}, and performance analysis \cite{darwish2022ste}\cite{uchida2021automated}\cite{istasse2019associative}\cite{theagarajan2020automated}.

                    %%%%%%%%%%%%%%%%%%%%%%%%%%
%-------------------%    TASK DESCRIPTION    %--------------------
                    %%%%%%%%%%%%%%%%%%%%%%%%%%

Explain why we need tracking for automated sport analysis.
Explain what is tracking and why it is challenging.
Explain re-identification is useful for solving the tracking task and why (because it helps capture the appearance of the player, and not lose its track when there is an occlusion or when he goes out of camera view)
Explain that further information is needed for automated analysis: team and role.
Gives examples of why tracking + id (reid)  + team + role is useful for downstream tasks.

% While recent work in pedestrian tracking has shown promising results by formulating multi-target tracking in terms of data association \cite{bewley2016simple}\cite{wojke2017simple}\cite{aharon2022bot}\cite{zhang2022bytetrack}\cite{du2023strongsort}\cite{cao2023observation}, player tracking in team sports presents unique challenges due to non-linear player motion, similar appearances of players on the field, and frequent occlusions. These challenges make it difficult to accurately track and re-identify players throughout the game. Therefore, re-identification plays a crucial role in player tracking and can significantly impact the accuracy of tracking methods. 

                    %%%%%%%%%%%%%%%%%%%%%%%%%%
%-------------------%       CHALLENGES       %--------------------
                    %%%%%%%%%%%%%%%%%%%%%%%%%%

Comments:
Crucial part: readers understand the context and that automated sport analysis = tracking + reid + role + team.
Now they need to understand how it has been done before, why it's not perfect or why there are some missing points, and why it's challenging.
Here we need to give an overview of what exists and why it's not the best solution.
Then we will introduce our solution in the next paragraph.

OVerview of the text to be written here:

Explain that most current tracking methods in the literature do not solve all these tasks at once (cite many sport tracking paper)
Explain that these tasks are generally solved by multiple networks with independent backbones, which is 1) compute intensive and therefore problematic for real-time applications, and 2) not optimal since all three concern sport person representation and are therefore closely related.
Explain role classification is generally solved by the upstream object detector, but most SOTA pre-trained  detectors are limited to the "person" class and cannot distinguish between various sports roles (cite a few of them, player, goalkeeper, referee, etc).
Explain team affiliation is formulated wrongly in most works (as classification task: cite/explain previous work), and that ReID models trained with identity labels cannot be used for team affiliation, as they might consider players with similar attributes other than the jersey color (e.g. skin color) more similar to each other than players from the same team.


% By accurately re-identifying players in soccer videos, tracking them becomes much easier. Although there has been a lot of research on re-identifying pedestrians \cite{fan2019spherereid}\cite{luo2019bag}, recently, part-based re-identification methods have gained attention due to their potential to localize different parts of a person and identify individuals using these parts \cite{sun2018beyond}\cite{xu2021dual}\cite{somers2023body}. These methods have shown promising results in dealing with the challenges such as occlusions. In addition, there have been several works that specifically focus on tracking and re-identification in sports \cite{liu2020part}\cite{maglo2022efficient}\cite{zhang2020multi}\cite{scott2022soccertrack}. However, a major challenge in this area has been the lack of a common dataset for evaluating and comparing different tracking and re-identification methods. To address this issue, the recently-introduced SoccerNet-Tracking dataset provides a common benchmark for evaluating player tracking and re-identification methods in soccer videos \cite{cioppa2022soccernet}.

                    %%%%%%%%%%%%%%%%%%%%%%%%%%
%-------------------%        SOLUTION        %--------------------
                    %%%%%%%%%%%%%%%%%%%%%%%%%%

Describe that, to face above issues, we propose a novel sports person representation model, that produces a multi-purpose representation from a single backbone: the extracted representation can be used to jointly solve the person re-identification, team affiliation and role classification tasks. 
Our method has two key benefits:
	1. By integrating three distinct representation objectives during training, the model generates richer representations, resulting in superior re-identification performance compared to a model trained with a single objective.
	2. It is compute efficient because it solves three tasks jointly with a single backbone
 3. Different from previous works (cite them), team affiliation is formulated as deep metric learning task, allowing the model to generalize to any team, and therefore be able to distinguish between two team it has not seen during training. 


                    %%%%%%%%%%%%%%%%%%%%%%%%%%
%-------------------%        APPROACH        %--------------------
                    %%%%%%%%%%%%%%%%%%%%%%%%%%

Describe that we start from BPBreID.
Describe very shortly BPBreID (body part-based method, sota).
Describe that we add two head on top of it: team affiliation and role classfication.
Describe role = classification task and team affiliation = clustering task.
Describe we train the model end to end as multi-task learning
Tell our model output part-based feature vector that can be used to solve the three tasks at inference.
Describe we test our sports person representation model within a sota tracking method: StrongSORT, and replace their spatio-temporal tracklet pose-processing step with a novel reid-based tracklet merging (explain shortly in the methodology what their AFLink module does and why we upgrade it with reid information)


                    %%%%%%%%%%%%%%%%%%%%%%%%%%
%-------------------%      CONTRIBUTIONS     %--------------------
                    %%%%%%%%%%%%%%%%%%%%%%%%%%

In summary, the main contributions of our work are as follows:

\begin{itemize}
\item We propose PRTreID, a novel multi-task sports person representation model to address re-identification, team affiliation, and role classification simultaneously. 
We demonstrate the benefit of multi-task learning to produce richer feature representations. 
To our knowledge, we are the first to address these three significant representation tasks with a single model.

\item We propose a two-step tracking method based on our multi-task sports person representation model, that produces long-term tracks together with targets identities, roles and teams.

\item We introduce a novel sport person representation dataset derived from SoccerNet tracking.

\item We publicly release our codebase and dataset to encourage further research on joint representation learning for sport.

Finally, we conduct extensive experiments to validate the effectiveness of our proposed model for person re-identification, role classification, team affiliation and multi-person tracking, and to demonstrate the key benefit from multi-task learning.
 

\end{itemize}
